RINN: One Sample Radio Frequency Imaging based on Physics Informed Neural Network

Due to its ability to work in non-line-of-sight and low-light environments, radio frequency (RF) imaging technology is expected to bring new possibilities for embodied intelligence and multimodal sensing. However, widely used RF devices (such as Wi-Fi) often struggle to provide high-precision electromagnetic measurements and large-scale datasets, hindering the application of RF imaging technology. In this paper, we combine the ideas of PINN to design the RINN network, using physical constraints instead of true value comparison constraints and adapting it with the characteristics of ubiquitous RF signals, allowing the RINN network to achieve RF imaging using only one sample without phase and with amplitude noise. Our numerical evaluation results show that compared with 5 classic algorithms based on phase data for imaging results, RINN's imaging results based on phaseless data are good, with indicators such as RRMSE (0.11) performing similarly well. RINN provides new possibilities for the universal development of radio frequency imaging technology.

==> figures/pinn.tex <==


% NEURAL NETWORK with coefficients, no arrows
\begin{tikzpicture}[x=1cm,y=1cm]
    
    \message{^^JNeural network without arrows}
    \readlist\Nnod{2,5,5,5,1} % array of number of nodes per layer
    \def\xscale{0.9}
    \message{^^J  Layer}
    \def\inputvalues{{"x", "t"}} % input values array
    \def\pinnvalues{{"$\frac{\partial}{\partial x}$", "$\frac{\partial}{\partial t}$","$\frac{\partial^2}{\partial x^2}$"}} % input values array
    \def\NP{3} % number of nodes in input layers
    \foreachitem \N \in \Nnod{ % loop over layers
      \def\lay{\Ncnt} % alias of index of current layer
      \pgfmathsetmacro\prev{int(\Ncnt-1)} % number of previous layer
      \message{\lay,}
      \foreach \i [evaluate={\y=(\N/2-\i)*0.7; \x=\lay*\xscale; \n=\nstyle;}] in {1,...,\N}{ % loop over nodes
        
        % NODES
        \ifthenelse{\lay=1}{
            \node[node \n] (N\lay-\i) at (\x,\y) {\pgfmathparse{\inputvalues[\i-1]}\pgfmathresult};
            }{\ifthenelse{\lay=5}{
                \node[node \n] (N\lay-\i) at (\x,\y) {u};
            }{
                \node[node \n] (N\lay-\i) at (\x,\y) {};
            }}
        
        % CONNECTIONS
        \ifnum\lay>1 % connect to previous layer
          \foreach \j in {1,...,\Nnod[\prev]}{ % loop over nodes in previous layer
            \draw[connect,white,line width=1.2] (N\prev-\j) -- (N\lay-\i);
            \draw[connect] (N\prev-\j) -- (N\lay-\i);
            %\draw[connect] (N\prev-\j.0) -- (N\lay-\i.180); % connect to left
          }
        \fi % else: nothing to connect first layer
        
      }
    }
    
    % LABELS
    \node[above=5,align=center,mygreen!60!black] at (N1-1.90) {input\\};
    \node[above=2,align=center,gray] at (N3-1.90) {hidden layer};
    \node[above=8,align=center,myblue!60!black] at (N\Nnodlen-1.90) {output};
    
    \foreach \i [evaluate={\c=int(\i==\NP); \y=\NP/2-\i;;}]
              in {1,...,\NP}{ % loop over nodes
    \node[node pinn] (NP-\i) at (6*\xscale,\y) {\pgfmathparse{\pinnvalues[\i-1]}\pgfmathresult};
    \draw[connect arrow] (N5-1) -- (NP-\i);
  }

  \node[align=left,myorange,fill=myorange!20!white](pinn_euq) at (7,-0.5) {$\frac{\partial u}{\partial t}+u\frac{\partial u}{\partial x}$\\$=v\frac{\partial^2 u}{\partial x^2}$};
  \draw[connect arrow,out=0,in=120] (NP-1) to (pinn_euq.north);
  \draw[connect arrow] (NP-2) to (pinn_euq.west);
  \draw[connect arrow,out=0,in=-120] (NP-3) to (pinn_euq.south);

  \end{tikzpicture}
  

==> figures/step.tex <==
\begin{tikzpicture}[every node/.style = {
    thick,
    rectangle, 
    draw,
    text width = 55, 
    minimum height = 12,
    align=center
    }]
  
\node[draw, rounded corners,align=center,fill=mygreen!25](pre) at (0,0) {Preprocessing\\(Sec.~\ref{sec:preprocessing})};
\node[draw, rounded corners,align=center,below of =pre](coor) {Coordinat\\ information};
\node[draw, rounded corners,align=center,fill=myblue!20](pinn) at (3,-0.5) {WINN\\(Sec.~\ref{sec:network})};
\node[draw, rounded corners,align=center,fill=myred!20](task) at (6,-0.5) {Result processing\\(Sec.~\ref{sec:task})};

\draw[-stealth,out=0,in=180] (pre) to  node[above,draw=none]{$\hat{\bm{E}}_s$} (pinn);
\draw[-stealth,out=0,in=180] (coor) to  node[below,yshift=-5,draw=none]{$\bm{E}_i, \bm{X}$} (pinn);
\draw[-stealth] (pinn) to node[above,draw=none]{$\bm{\varepsilon}$} (task);
\node[fit=(pre)(coor)(pinn)(task),draw,inner sep=3pt]{};
\end{tikzpicture}

==> sections/design.tex <==
\section{System design}
\begin{figure*}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/overview.pdf}
    \caption{WINN}
    \label{fig:winn}
\end{figure*}
% \begin{figure}
%     % \resizebox{\linewidth}{!}{\input{figures/step.tex}}
%     \input{figures/step.tex}
%     \caption{Overview}
%     \label{fig:over}
% \end{figure}

% Fig.~\ref{fig:over} illustrates the fundamental workflow of the system for sensing, which primarily comprises three components: preprocessing (Sec.~\ref{sec:preprocessing}), the Wireless-informed Neural Network (WINN) (Sec.~\ref{sec:network}), and result processing (Sec.~\ref{sec:task}).
In the preprocessing stage, we estimate the scattered wave \(\hat{E}_s\) using the received signal at the receiver and obtain an estimate of the incident wave \(E_i\) by leveraging the position of the transmitter and the basic characteristics of electromagnetic wave propagation. These estimates, along with the coordinates $\bm{X}$ of the discretized sensing area \(\mathcal{D}\), are fed into the WINN.
We design this perception network by integrating the concept of PINN, embedding the physical laws governing wireless signal propagation to estimate the complex permittivity from phaseless data.
This network benefits from the nonlinearity of neural networks and converges based on actual physical constraints rather than requiring large amounts of training data.
% Finally, in the result processing stage, we extract the shape and material properties of the target from the distribution of the complex permittivity.


\subsection{Preprocessing}
\label{sec:preprocessing}
To utilize WiFi data for material identification in field sensing models, we need to address two primary issues: \textbf{data noise} and \textbf{gain differences}. For the amplitude data, which is relatively stable and suitable for our subsequent tasks, we focus on reducing noise by applying mean filtering and removing outliers from the raw data. Additionally, because our system employs multiple independent transmitters and receivers, these devices might introduce varying signal gains. 
Handling these gain differences is crucial for ensuring consistent and reliable material identification.

\begin{figure}
	\subfloat[]{\includegraphics[width=0.47\linewidth]{figures/abs.pdf}}
	\hfill
	\subfloat[]{\includegraphics[width=0.47\linewidth]{figures/phase.pdf}}
	\caption{The amplitude of WiFi signals is more stable than the phase after smoothing. (a) Amplitude. (b) Phases.}
	\label{fig:signal}
\end{figure}

The received signal $R$ is the result of electromagnetic waves transmitted in space after undergoing processes such as antenna gain and automatic gain control (AGC).
Additionally, it is subject to zero-mean Gaussian noise~\cite{terryOFDMWirelessLANs2003}, which can be represented as:
\begin{equation}
    R = G_{agc} G_{ant} E_t + N,
\end{equation}
where \(G_{agc}\) and \(G_{ant}\) are the AGC gain and antenna gain, respectively; \(E_t\) is the electric field; and \(N\) is the noise.

Since Gaussian noise has a zero mean, we use the expectation of the received signal for subsequent processing.
Fig.~\ref{fig:signal} shows the signal after taking the expectation, revealing that the amplitude exhibits good stability.
However, due to the presence of modulus operation, if the phase error range of the device itself is large, the expected value is not stable.
Therefore, in the subsequent processing, we only use the amplitude of the received signal.
Moreover, the AGC $G_{agc}$ of WiFi devices can be obtained.
Therefore, the issue now lies solely in how to eliminate the impact of antenna gain \( G_{ant} \) differences.
Fortunately, \( G_{ant} \) is only related to the device itself, and we can obtain it through a preliminary calibration, which is given by:
\begin{equation}
    G_{ant} = \mathbb{E} \left[\frac{R_{w/o}}{G_{agc} E_t}\right],
\end{equation}
where \( R_{w/o} \) is the received signal without the target, and \( \mathbb{E} \) denotes the expectation.
Since there is no scattered wave from the target at this time, the total electric field is equivalent to the incident wave. According to the propagation characteristics of electromagnetic waves, it is:
\begin{equation}
    E_t = E_i = \frac{e^{j\omega t}}{r},
    \label{eq:incident}
\end{equation}
where \( r \) is the distance between the transmitter and the receiver and \( \omega \) is the angular frequency.

\subsection{WINN}
\label{sec:network}


Unlike many artistic two-stage schemes, we do not have a large amount of labeled data for model training. 
Instead, we use the idea of PINN~\cite{zhengImplementationMaxwellsEquations2024} to try to train a regression network so that the output of the network can satisfy Equ.~\ref{eq:model-d} for the current input signal. 
In this way, we achieve "single-sample sensing".
However, due to having only one sample of input data, it is very easy for the network to overfit.
Inspired by research~\cite{song2021scorebasedgenerativemodelingstochastic}, we view the network as a mapping between two random variables rather than between two numerical values.
The overall framework of WINN is illustrated in Fig.~\ref{fig:winn}.
Specifically, we designed two multilayer perceptrons (MLP), whose outputs represent the mean values of complex dielectric constant and induced current, and then used Equ.~\ref{eq:model-d} as a physical constraint to achieve regression.
As a result, we obtain the solution under the current received signal conditions.

\subsubsection{$\varepsilon$-MLP}
We use $\bm{\varepsilon}$-MLP with parameters $\theta_{\varepsilon}$ to map the spatial coordinates $x$ of the sensing area $\mathcal{D}$ to their associated complex permittivity.
We assume that the output $\bm{\varepsilon}$ of the network is a Gaussian random variable, i.e., $\bm{\varepsilon} \sim \mathcal{N}(\mu_{F_\varepsilon},\Sigma_{\varepsilon})$. 
We use the $\varepsilon$-MLP network to represent a probability mapping $p_{\theta_{\varepsilon}}(\varepsilon|x)$.
The output of the $\varepsilon$-MLP is:
\begin{equation}
    \bm{F_\varepsilon} = F_{\varepsilon}(\bm{X};\theta_{\varepsilon}).
    \label{eq:epsilon-mlp}
\end{equation}

A noteworthy detail is that we perform random resampling on the discretized sensing area $\mathcal{D}$ to obtain the input $X$ for the $\varepsilon$-MLP.
Specifically, we first discretize the sensing area $\mathcal{D}$ into an $N$ grid\footnote{Regardless of the shape of the sensing region D, we can always enclose it with a rectangle. Since we are only concerned with targets outside the air, this does not affect the sensing outcomes.}, with the center coordinates of each grid being $X^{\mathcal{D}}$.
Then, a zero-mean Gaussian random variable is added to each grid center coordinate to obtain the random coordinate $X$, i.e., 
\begin{equation}
    X_{i} = X^{\mathcal{D}}_{i} + n_{\mathcal{D}},
\end{equation}
where \(X_{i}\) and \(X^{\mathcal{D}}_{i}\) are the $i$-th element of $X$ and $X^\mathcal{D}$, respectively, and \(n_\mathcal{D} \sim \mathcal{N}(0,\sigma^2) \) is a Gaussian random variable.
The introduction of random resampling endows the $\varepsilon$-MLP with the capability to represent continuous functions, which helps to present imaging details at a finer granularity.
On the other hand, random resampling does not alter the shape of $X^\mathcal{D}$, and $X$ and $X^\mathcal{D}$ have the same expectation, making it compatible with classical numerical computation schemes for electromagnetic waves, facilitating the construction of the loss function based on Equ.~\ref{eq:model}.

\subsubsection{J-MLP}
After obtaining the complex permittivity \(\bm{\varepsilon}\), the induced current \(\bm{J}\) can be obtained by solving Equ.~\ref{eq:models} and Equ.~\ref{eq:current} simultaneously, which subsequently allows for the derivation of the scattered wave \(E_s\).
However, this process involves matrix inversion, which is computationally intensive and poses challenges for gradient calculation.
Therefore, we designed a $\bm{J}$-MLP network $F_J$ to obtain the induced current \(\bm{J}\) without performing matrix inversion.
Similar to $\varepsilon$-MLP, $J$-MLP is also not a one-to-one mapping of numbers. 
We assume its output $\bm{J}$ is a Gaussian random variable, that is, $J \sim \mathcal{N}(\mu_{F_J},\Sigma_J)$.
J-Net acts as an encoder to represent a probability mapping $p_{\theta_J}(J|x,E_i)$.
The output of the $J$-MLP is:
\begin{equation}
    \bm{F_J} = F_{J}(X,\bm{E}_i;\theta_{J}),
    \label{eq:J-mlp}
\end{equation}
where $\bm{E}_i$ is the incident wave in the sensing domain $\mathcal{D}$ which is given by Equ.~\ref{eq:current-d}, $\bm{X}$ is the spatial coordinates of the sensing area $\mathcal{D}$, and $\theta_{J}$ are the parameters of the $\bm{J}$-MLP.

\begin{figure*}
    \centering
    \subfloat{\includegraphics[width=0.95\linewidth]{figures/gt.pdf}}

    \subfloat{\includegraphics[width=0.95\linewidth]{figures/res.pdf}}
    \caption{The workflow of the system for sensing.}
    \label{fig:step}
 \end{figure*}
\subsubsection{Loss function}
When the network converges, we aim to: (1) make the scattered wave corresponding to the complex permittivity as close as possible to the actual measured data, and (2) ensure that the induced current in the sensing domain $\mathcal{D}$ satisfies the constraints of equation Equ.~\ref{eq:model}.
To achieve these goals, we have designed a \emph{scatter loss} $\mathcal{L}_{sa}$ and a \emph{sensing domain loss} $\mathcal{L}_\mathcal{D}$ to constrain each part, addressing the practical issues mentioned in Sec.~\ref{sec:practical}.
 

\textbf{Scatter loss.} 
An intuitive design is to multiply the output of the J-MLP—induced current \( \bm{F}_{J} \)—with \( G_s \) to obtain the scattered wave, then extract the corresponding scattered signal from the received signal to compute their MSE loss.
However, due to the lack of phase data and the fact that the received signal is a superposition of the incident and scattered waves, we define the scattering loss as:
\begin{equation}
    \begin{aligned}
         \mathcal{L}_{sa} &= \left| \Vert \bm{G}_s \bm{\mu}_{J} + \bm{E_i^R} \Vert - \Vert \hat{\bm{E}}_t \Vert \right|_2\\
            &= \mathbb{E}\left(\left| \Vert \bm{G}_s \bm{F_J} + \bm{E_i^R} \Vert - \Vert \hat{\bm{E}}_t \Vert \right|_2\right)
    \end{aligned}
    \label{eq:scatter}
\end{equation}
where \( \bm{E_i^R} \) is the incident wave in the receivers, and \( \hat{\bm{E}}_t \) is the received signal after preprocessing, $\Vert \cdot \Vert$ is the amplitude operation, and \( | \cdot |_2 \) is the Euclidean norm, and $\mathbb{E}$ means expectation.

\textbf{Sensing domain loss.}
To train the $\varepsilon$-MLP, we designed a perception region loss.
Specifically, the induced current \( \bm{J} \) has two representations, given by Equ.~\ref{eq:model-d} and Equ.~\ref{eq:J-mlp}.
Theoretically, these two should be identical.
Therefore, \( \mathcal{L}_{\mathcal{D}} \) is designed as follows:
\begin{equation}
    \begin{aligned}
        \mathcal{L}_{\mathcal{D}} &= \left| \bm{\mu_J} - [Diag(\bm{\mu_\epsilon})-1](\bm{E}_i + \bm{G}_\mathcal{D}\bm{\mu_J})\right|_2\\
        &= \mathbb{E}\left(\left| \bm{F_J} - [Diag(\bm{F_\epsilon})-1](\bm{E}_i + \bm{G}_\mathcal{D}\bm{F_J})\right|_2\right)
    \end{aligned}
    \label{eq:sensing}
\end{equation}
where \( Diag(\bm{F_\epsilon}) \) is a diagonal matrix with the elements of \( \bm{F_\epsilon} \) on the diagonal.



As  a result, the total loss function is:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{sa} + \lambda \mathcal{L}_{\mathcal{D}},
    \label{eq:total}
\end{equation}


\subsection{Implementation}
We use Julia scripts for data processing, and implement the WINN network using the Lux.jl library~\cite{pal2023efficient,pal2023efficient}.
Two eight-layer MLPs with 64 channels and ReLU activation each are used to predict $\bm{F}_{\varepsilon}$  and $\bm{F}_{J}$.
During training, the sensing sensing $\mathcal{D}$ is discretized into 4096 sub-regions of size 64 $\times$ 64. The hyperparameters setting for overall loss is $\lambda = 1.00$.
 We use Adam optimizer with default values, learning rate of $5\times 10^{-4}$, decayed during optimization process following an exponential scheduler.
 The batch size of input networks is set to be 64. 
 We train the WINN network on NVIDIA GTX4090 GPU.

% \subsection{Result processing}
% \label{sec:task}
% Edge detection in images is commonly employed to differentiate objects from their surroundings. This technique operates under the premise that the variation among pixel values within the object (or target) area and within the background area is relatively minor, whereas there is a significant shift in pixel values at the boundary where the object meets the background.
% At these edges, there's a pronounced 'leap' or substantial alteration in pixel intensity. Consequently, the first derivative of pixel values along an edge exhibits a peak, while the second derivative crosses zero at these points. Leveraging these characteristics, algorithms can effectively identify and delineate edges within an image.

% For edge detection, we employ the Canny operator. Initially, we apply Gaussian filtering to the image to reduce noise. Following this, the Canny operator is used to compute the gradient magnitude \( U(x, y) \) and the gradient direction \( \theta_u(x, y) \) at each point in the image, which are given by:
% \begin{equation}
%     \begin{aligned}
%         &U(x,y) =\sqrt{U_{x}^{2}(x,y)+U_{y}^{2}(x,y)}, \\ 
%         &\theta_u(x,y) =\arctan \left(\frac{U_{y}(x,y)}{U_{x}(x,y)}\right),\\
%     &U_x=\left[\begin{array}{ll}
%     1 & -1 \\
%     1 & -1
%     \end{array}\right],\quad U_y=\left[\begin{array}{cc}
%     -1 & -1 \\
%     1 & -1
%     \end{array}\right]
%     \end{aligned}
% \end{equation}
% where $U_{x}(x,y)$ and $U_{y}(x,y)$ are the horizontal and vertical gradients of the image, respectively.
% After applying non-maximum suppression to the gradient image \( U(x, y) \), we use a thresholding technique to identify the edges.
% Specifically, each pixel is compared with its two neighbors in the direction of the gradient.
% If the gradient value of the pixel is not the highest among these three, it is suppressed—set to zero. Finally, the edge positions are determined based on the threshold values.

% Given that the complex permittivity differs among various liquids, the final imaging results show distinct pixel values for different types of liquids. Therefore, we can extract the top \( k \) values as features representing the liquid from the imaging result. These features are then used with a k-nearest neighbor (KNN) classifier to identify the type of liquid.


==> sections/intro.tex <==
\section{Introduction}

Identifying the material and shape of targets is crucial for decision-making in many intelligent systems.
For example, it helps robots determine the appropriate force and posture to grasp objects and assists radar systems in distinguishing between birds and drones.
Due to their sensing capabilities under low-light or non-line-of-sight conditions, radio frequency (RF) signals offer unique advantages in various scenarios~\cite{chenWirelessSensingMaterial2024}.

Recently, numerous RF-based material identification systems (such as LiqDetector~\cite{wangLiqDetectorEnablingContainerIndependent2023}, LiqRay~\cite{shang2022liqray}, SoilCares~\cite{wangSoilCaresLowcostSoil2024}, and etc.) or imaging systems (such as Wi2DMeasure~\cite{wangWi2DMeasureWiFibased2D2024}, WiProfile~\cite{yaoWiProfileUnlockingDiffraction2024}, Wiffract~\cite{pallaproluWiffractNewFoundation2022}, and etc.) have been proposed; however, they often can only handle one sensing task at a time, either imaging or material identification.
WiPainter~\cite{yanWiPainterFinegrainedMaterial2023} proposed a system based on COTS WiFi devices that utilizes material polarization to achieve integrated material-imaging sensing.
However, it can only identify targets much larger than the wavelength, which limits the applicability of the most widely available wireless signals—sub-6 GHz signals—in many scenarios. 
LiquImager~\cite{shangLiquImagerFinegrainedLiquid2024}, based on Maxwell's equations, proposed a field sensing model capable of fine-grained sensing of near wavelength targets.
However, its reliance on data training poses a challenge, as collecting comprehensive and diverse RF datasets is difficult.

In summary, we have three objectives:
\begin{itemize}
    \item Integrated imaging-identification sensing. We aim for sensing results that not only provide information about the material or shape of targets but also offer a portrait-like characterization of the sensing area, encompassing both shape and material information of different shapes. 
    \item Near-wavelength target sensing. Given that many scenarios involve centimeter-scale targets, we aim to enable widely available centimeter waves, such as WiFi signals, to sense near-wavelength targets. 
    \item Unknown target sensing. The materials and shapes of targets in real-world sensing scenarios are highly varied, making it challenging to collect sufficiently rich RF datasets. We aim for the system to recognize targets not present in the dataset.
\end{itemize}

We no longer treat material identification and imaging as separate tasks but instead attempt to accomplish these two seemingly unrelated tasks within a single framework.
A fundamental insight stems from the fact that different materials possess distinct complex permittivity.
If we can reconstruct the complex permittivity distribution of the sensing area, these two sensing tasks are naturally completed: varying complex permittivity indicate different materials, while their boundaries reveal shape information.
LiquImager~\cite{shangLiquImagerFinegrainedLiquid2024} employs a field seising model based on Maxwell's equations to finely characterize the impact of complex permittivity on the received signals. However, two prominent challenges remain to be addressed.

(1) The combinations of different materials, shapes, and positions are so numerous that collecting a sufficiently rich training dataset is extremely challenging.
For a common scenario, such as identifying a beverage on a table, there can be dozens of possible locations, tens of material types, and numerous combinations of container shapes and sizes, leading to tens of thousands of total possibilities. Given the difficulty in collecting radio frequency data, constructing a sufficiently diverse dataset for material identification using machine learning classification is challenging.

(2) The number of parameters to be estimated is large, while the amount of directly measurable data is scarce and highly noisy. Our goal is to estimate the distribution of the complex dielectric constant in the sensing area. Even for a desktop-sized region (a few square meters), discretization can result in tens of thousands of parameters to be estimated \footnote{To image objects at the centimeter level, the grid size is typically set to \qty{1}{cm} or smaller.}. However, the signals we can collect are limited to data from a few transceiver antennas; for example, the Intel 5300 network card has only three antennas, providing just nine antenna pair data combinations in a one-to-one transmit-receive configuration. Moreover, WiFi data contains significant noise due to issues such as imprecise clock synchronization, which further complicates parameter estimation.

Our Solutions. Unlike traditional methods that first use physical models for preprocessing and then enhance the results with deep learning networks, we aim to leverage the inherent physical constraints of Maxwell's equations to design network constraints. This leads to the construction of a physics-informed deep learning network that performs sensing tasks in an unsupervised manner. Furthermore, we utilize physical relationships to estimate parameters that are difficult to measure directly and have developed a maximum likelihood optimization scheme to estimate parameters using phaseless data, addressing the issue of severe phase noise.

==> sections/overview.tex <==



==> sections/pre.tex <==
\section{Preliminaries}

\subsection{Maxwell's equations}


Material identification and imaging using RF signals stem from a fundamental observation: the distribution of complex permittivity in space affects the propagation of RF signals, which is described by Maxwell's equations~\cite{IntroductionToElectrodynamics}.
For a medium that is uniform in the $z$-direction with the electric field having only a $z$-component, Maxwell's equations can be simplified to
\begin{equation}
    \frac{\partial^2 E}{\partial x^2} + \frac{\partial^2 E}{\partial y^2} + k^2 E = 0
    \label{eq:maxwell}
\end{equation}
where $E$ is the electric field, $(x,y)$ is the position, and $k$ is the wavenumber that is related to the complex permittivity.

\subsection{Physics-informed neural networks}

\begin{figure}
    \resizebox{\linewidth}{!}{\input{figures/pinn.tex}}
    \caption{The electric field $\vec{E}$ and the magnetic field $\vec{B}$ are perpendicular to each other and to the direction of propagation of the wave.}
    \label{fig:pinn}
\end{figure}

The physics-informed neural network (PINN) model typically consists of a deep neural network, characterized by the inclusion of a physics-informed term in the loss function, representing the physical laws to be followed~\cite{karniadakisPhysicsinformedMachineLearning2021}. For instance, in fluid dynamics, the Navier-Stokes equations might be used as the physical information. During training, the model not only minimizes data error but also reduces the error associated with the physics-informed term, ensuring that the predictions adhere to physical laws.

In traditional machine learning approaches, the learning process is primarily data-driven, with models heavily relying on large amounts of high-quality data. However, in practical applications, data scarcity or noisy data often pose significant challenges. Under such circumstances, data-driven models alone struggle to produce accurate and reliable predictions. In contrast, PINNs (Physics-Informed Neural Networks) incorporate physical knowledge as a prior, aiming to overcome the limitations of insufficient data. By leveraging physical laws, PINNs can provide physically intuitive predictions even when data are limited.

A simple example is illustrated in Fig.~\ref{fig:pinn} where we consider the Burgers' equation, \(\frac{\partial u}{\partial t}+u\frac{\partial u}{\partial x}=v\frac{\partial^2 u}{\partial x^2}\).
 We take the two independent variables, \(x\) and \(t\), of the differential equation as inputs to a Multi-Layer Perceptron (MLP), and regard the output of the MLP as the dependent variable \(u\) of the equation.
 Subsequently, using the automatic differentiation mechanism of neural networks, we obtain the partial derivatives of \(u\) with respect to \(x\) and \(t\), denoted as \(\frac{\partial u}{\partial x}\), \(\frac{\partial u}{\partial t}\), and \(\frac{\partial^2 u}{\partial x^2}\). The loss function is derived from the physical equation itself, for instance, it could be
 \begin{equation}
    \mathcal{L} = \sum \left(\frac{\partial u}{\partial t}+u\frac{\partial u}{\partial x}-v\frac{\partial^2 u}{\partial x^2}\right)^2.
 \end{equation}
  When the loss function converges to a very small value, we naturally obtain an approximate solution to the equation. Unlike traditional training schemes that rely on comparing predicted values with labels, the training of PINNs is based on physical constraints rather than large datasets.
  This concept inspires us to design a non-data-driven target-aware scheme.
